LearnedWMP: Workload Memory Prediction Using Distribution of Query Templates

In a modern DBMS, working memory is frequently the limiting factor when processing in-memory analytic query operations such as joins, sorting, and aggregation. Existing resource estimation approaches for a DBMS estimate the resource consumption of a query by computing an estimate of each individual database operator in the query execution plan. Such an approach is slow and error-prone as it relies upon simplifying assumptions, such as uniformity and independence of the underlying data. Additionally, the existing approach focuses on individual queries separately and does not factor in other queries in the workload that may be executed concurrently. In this research, we are interested in query performance optimization under concurrent execution of a batch of queries (a workload). Specifically, we focus on predicting the memory demand for a workload rather than providing separate estimates for each query within it. We introduce the problem of workload memory prediction and formalize it as a distribution regression problem. We propose Learned Workload Memory Prediction (LearnedWMP) to improve and simplify estimating the working memory demands of workloads. Through a comprehensive experimental evaluation, we show that LearnedWMP reduces the memory estimation error of the state-of-the-practice method by up to 47.6%. Compared to an alternative single-query model, during training and inferencing, the LearnedWMP model and its variants were 3x to 10x faster. Moreover, LearnedWMP-based models were at least 50% smaller in most cases. Overall, the results demonstrate the advantages of the LearnedWMP approach and its potential for a broader impact on query performance optimization.

==> experiments.tex <==
%\section{Experimental Evaluation}
%\label{sec:evaluation}

We experimentally evaluated the performance of our proposed LearnedWMP model for the workload memory prediction problem. Then, we evaluate different variants of LearnedWMP, different parameters, and different components, such as learning query template techniques (see section \ref{subsection:learning-query-templates}). In this section, we describe the experimental setup and then present the experiment results. 

\subsection{Experiment Setup} 
%We describe the experimental setup, dataset, metrics, and LearnedWMP variations. 
\stitle{Environment.} We conducted the experiments using a commercial DBMS instance running on a Linux system with 8 CPU cores, 32 GB of memory, and 500 GB of disk space. 

\stitle{Workload Datasets.} We used three popular database benchmarks: \texttt{TCP-DS}\cite{nambiar2006making} %\footnote{\url{https://www.tpc.org/tpcds/}},
\texttt{Join Order Benchmark} or \texttt{JOB} \cite{leis2015good}, and \texttt{TPC-C}\cite{leutenegger1993modeling}. \texttt{TPC-DS} and \texttt{JOB} are benchmarks for {\em analytical workloads}, whereas \texttt{TPC-C} is for {\em transactional workloads}. We used either its query generation toolkit or the seed query templates for each benchmark to generate queries for our experiment. We generated 93000 queries for \texttt{TPC-DS}, 2300 queries for \texttt{JOB}, and 3958 queries for \texttt{TPC-C}. For each benchmark, we randomly divided the queries into training ($\mathcal{Q}_{train}$) and test ($\mathcal{Q}_{test}$) partitions, with 80\% of the queries belonging to $\mathcal{Q}_{train}$ and the remaining 20\% to $\mathcal{Q}_{test}$. We grouped queries into workload batches from training and test partitions. We experimented with different batch sizes and found 10 to be a decent size to improve the memory estimation of our experimental workloads. We discuss our experiment with batch size parameter in section \ref{sec:effect-of-batch-size}.

\stitle{Methods} In the workload memory prediction problem, we aim to estimate the aggregate memory utilization of a query batch (i.e., workload). As there are no existing libraries or methods for this novel problem, we develop and evaluate different variants of LearnedWMP and compare them with available baselines to assess their performance. %we are interested in the aggregate estimation of memory utilization of a batch of queries (i.e., a workload). Since this is a novel problem, there are not any off-the-shelf libraries or state-of-the-art methods in the literature that we could employ in the comparative performance analysis of our method. We, therefore, rely on the design, development, and evaluation of plausible variants of LearnedWMP and available baselines for addressing the same problem.
% text wrap: https://tex.stackexchange.com/questions/111948/what-is-a-overfull-hbox-9-89561pt-too-wide

\smallskip \noindent \textbf{LearnedWMP-based Methods}. LearnedWMP accepts as input a workload $w$ and returns the workload's estimated working memory demand, $\hat{y}$. As described in section \ref{sec:other-ml-methods}, besides the proposed MLP-based deep neural network (DNN) method, we can use other ML techniques to learn the memory estimation regression function. Thus, we explored additional ML techniques, such as Ridge, DT, RF, and XGB, in this experiment. We refer to the LearnedWMP-based models trained with different ML techniques as \textit{LearnedWMP-DNN}, \textit{LearnedWMP-Ridge}, \textit{LearnedWMP-DT}, \textit{LearnedWMP-RF}, and \textit{LearnedWMP-XGB}. 


\begin{figure*}[t!]
  \makebox[\linewidth][c]{%
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCDS-RMSE Error.png}
         \caption{\texttt{TPC-DS}}
         \label{fig:TPC-DS-rmse}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/JOB-RMSE Error.png}
         \caption{\texttt{JOB}}
         \label{fig:JOB-rmse}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCC-RMSE Error.png}
         \caption{\texttt{TPC-C}}
         \label{fig:TPC-C-rmse}
     \end{subfigure}
     }
        \caption{Root Mean Squared Errors (smaller is better)}
        \label{fig:model-training-rmse}
        \vspace{-10px}
\end{figure*}

\smallskip \noindent \textbf{SingleWMP-based Methods}. An alternative approach to estimate the aggregate working memory demand of a workload is to rely on single-query-based memory predictions. In this approach, first, the highest working memory requirement for each query in the workload is estimated separately. Then these individual estimates are summed up to produce the aggregate working memory estimation for the workload. We refer to this method as \underline{Single}-query based \underline{W}orkload \underline{M}emory \underline{P}rediction (SingleWMP). Formally, given a workload $w$, consisting of a set of $\mathcal{Q}$ queries, the estimated working memory demand $\hat{y}$ of $w$ is:
\begin{equation}
\hat{y}=\sum_{i=1}^\mathcal{|Q|}{\hat{y}_{q_i}}
\end{equation}
where $\hat{y}_{q_i}$ is the estimated memory demand of a single query $q_i \in \mathcal{Q}$. In this approach, we use query plan features of each query as direct input to an ML algorithm. During the training phase, the algorithm additionally receives the historical memory utilization of each training query. Using the pairs of query plan features and memory utilization of many individual training queries, the algorithm learns a function to estimate the memory demand of individual queries. Unlike the LearnedWMP approach, the SingleWMP approach doesn't learn query templates from historical queries. Similar to LearnedWMP, we use DNN, Ridge, DT, RF, and XGB techniques to train five variations of the SingleWMP ML models. We refer to these variants of SingleWMP as \textit{SingleWMP-DNN}, \textit{SingleWMP-Ridge}, \textit{SingleWMP-DT}, \textit{SingleWMP-RF}, and \textit{SingleWMP-XGB}. An additional method of the SingleWMP approach is \textit{SingleWMP-DBMS} which obtains the estimated memory utilization for each query directly from a DBMS's query optimizer. SingleWMP-DBMS doesn't use ML in the memory estimation; instead, it relies on heuristics written by database experts. SingleWMP-DBMS represents {\em the current state of practice} in the commercial database management systems.
    
% \begin{sloppypar}
% \begin{itemize}
%     \item \textit{LearnedWMP-based Methods}. LearnedWMP accepts as input a workload $w$ and returns the workload's estimated memory demand, $\hat{y}$. As described in section \ref{sec:other-ml-methods}, besides the proposed MLP-based deep learning method (MLP), we can use other ML techniques to learn the memory estimation regression function. As additional ML techniques, in this experiment, we explored Ridge, DT, RF, and XGB. We refer to the LearnedWMP-based models trained with different ML techniques as \textbf{LearnedWMP-MLP}, \textbf{LearnedWMP-Ridge}, \textbf{LearnedWMP-DT}, \textbf{LearnedWMP-RF}, and \textbf{LearnedWMP-XGB}. 
%     \item \textit{SingleWMP-based Methods}. An alternative approach to estimate the aggregate memory demand of an workload is to rely on single-query based memory predictions. In this approach, first the memory requirement for each query in the workload is estimated separately, and then the single-query estimates are summed up to produce the aggregate memory estimation for the workload.
%     %Latter estimates the memory demand of each query in the workload batch separately and then sum up the estimates of all queries to produce as aggregate memory demand for the workload. 
%     We call this alternative approach a \underline{Single}-query based \underline{W}orkload \underline{M}emory \underline{P}rediction (SingleWMP) method. Formally, given a workload $w$, which consists of a set of $\mathcal{Q}$ queries, the estimated memory demand $\hat{y}$ of $w$ will be given by:
%     \begin{equation}
%     \hat{y}=\sum_i{\hat{y}_{q_i}}
%     \end{equation}
%     where $\hat{y}_{q_i}$ is the estimated memory demand of a single query $q_i \in \mathcal{Q}$. In this approach, we use query plan features of each query as direct input to an ML algorithm. During the training phase, the algorithm additionally receives the historical memory utilization of each training query. Using the pairs of query plan features and memory utilization of many individual training queries, the algorithm learns a function to estimate the memory demand of individual queries. Unlike the LearnedWMP approach, SingleWMP approach doesn't learn query templates from historical queries. Similar to LearnedWMP, we use MLP, Ridge, DT, RF, and XGB techniques to train five variations of the SingleWMP ML models. We refer to these variants of SingleWMP as \textbf{SingleWMP-MLP}, \textbf{SingleWMP-Ridge}, \textbf{SingleWMP-DT}, \textbf{SingleWMP-RF}, and \textbf{SingleWMP-XGB}. An additional method of the SingleWMP approach is \textbf{SingleWMP-DBMS} that obtains the estimated memory utilization for each query directly from a DBMS's query optimizer. \textbf{SingleWMP-DBMS} doesn't use ML in the memory estimation; instead, it relies on heuristics, written by database experts. \textbf{SingleWMP-DBMS} represents {\em the current state of practice} in a commercial database management system.
% \end{itemize}
% \end{sloppypar}

%\textbf{Accuracy Metrics:}
\stitle{Evaluation metrics} To evaluate the accuracy performance of various models, we use two accuracy metrics:
%We compared the memory estimation accuracy of all the models in two different levels: (1) between ML and Non-ML methods and (2) between LearnedWMP and Query-based ML models. In this comparison, we use the following two metrics:
\begin{itemize}
    \item Root Mean Squared Error (RMSE): For measuring the accuracy performance of the models --- LearnedWMP and SingleWMP --- we use $L_2$ loss or root mean squared error (RMSE), as follows:
    \begin{align}
    RMSE =  \sqrt{ \frac{\sum_{i=1}^N {(y_i-\hat{y_i})^2}}{N} }
    \label{eqmse}
    \end{align}
We seek to find an estimator that minimizes the RMSE.
\item IQR and Error Distribution: While RMSE is convenient to use, it doesn't provide insights into the distribution of prediction errors of a model. Two models can have similar RMSE scores but different distributions of errors. For each benchmark, we compute the signed differences between the actual and the predicted memory estimates - the residuals of errors. We use the residuals to generate violin plots, which help us compare the interquartile ranges (IQR) and the error distributions of different models. IQR is defined as follows \cite{dekking2005modern}.
    \begin{equation}
    IQR = q_n(0.75) - q_n(0.25)
    \end{equation}
    Here, $q_n(0.75)$ is the 75th percentile or the upper quartile, and the $q_n(0.25)$ is the 25th percentile or the lower quartile. The range of values that fall between these two quartiles is called the interquartile range (IQR). IQR is shown as a thick line inside the violin in a violin plot. A white circle on the IQR represents the median. When a model's violin is closer to zero and has a smaller violin, it is more accurate. 
\end{itemize}
In addition to computing accuracy, for each ML-based LearnedWMP and SingleWMP model, we measured the {\em model size} in kilobyte ($kB$), the {\em training time} in millisecond ($ms$), and the inference time in microsecond ($\mu$).

\subsection{Experiment Results and Discussion}

%\medskip\noindent\textbf{Scenarios}. With the above experiment setup, we explore answers to the following questions:
We evaluate the following aspects of the LearnedWMP model.
\begin{itemize}
\item \textbf{LearnedWMP accuracy performance}. How does the accuracy of LearnedWMP-based models compare to that of SingleWMP-based models?
%\item \textbf{LearnedWMP accuracy performance}. What is the accuracy performance of LearnedWMP-based models compared to SingleWMP-based models?

\item \textbf{LearnedWMP training and inference cost}. What is the runtime cost of training LearnedWMP-based models, and how does it compare to SingleWMP-based models'? What is the runtime cost of these models at the inference time?  

%\item \textbf{LearnedWMP model size}. What is the model size of the LearnedWMP-based models and how they compare to those of the SingleWMP-based models?
\item \textbf{LearnedWMP model size}. How does the size of the LearnedWMP-based models compare to that of the SingleWMP-based models?

\item \textbf{Learning query templates}. How does LearnedWMP's method for learning query templates compare to alternatives for improving the accuracy of workload memory estimation?

\item \textbf{Effect of the number of query templates}. What is the effect of the number of query templates $K$ on the memory estimation accuracy of the LearnedWMP models?

\item \textbf{Effect of the batch size parameter $s$}. What is the effect of batch size parameter $s$ on the memory estimation accuracy of the LearnedWMP models?

%\item \textbf{Q4 Comparative analysis of strategies for learning query templates} How LearnedWMP's method for learning query templates compares to  alternatives, in terms of improving the accuracy of workload memory estimation?
\end{itemize}
While comparing the LearnedWMP-based approach with the SingleWMP-based approach, we use accuracy, training time, inference latency, and the model size during the comparison. All these metrics are important when considering embedding an ML model in a commercial DBMS product.

% \begin{itemize}
% \item \textbf{Q1. Accuracy of the ML-based Memory Estimation Models} Are ML-based memory estimates more accurate than the state-of-the-art in a DBMS?
% \item \textbf{Q2. Efficiency of batch memory estimation} Is batch memory estimation more efficient than estimating the memory of each query separately?
% \item \textbf{Q3. Comparative analysis of strategies for learning query templates} For improving the accuracy of memory estimation, how effective is LearnedWMP's templatization method as compared to four alternate query templatization methods?
% \end{itemize}

%\subsection{Accuracy of the ML-based Memory Estimation Models}

%\subsection{LearnedWMP Accuracy Performance}

\begin{figure*}[t!]
     \centering
     \makebox[\linewidth][c]{%
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/tpcds_violinplot.png}
         \caption{\texttt{TPC-DS}}
         \label{fig:TPCDS-mtl}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/job_violinplot.png}
         \caption{\texttt{JOB}}
         \label{fig:JOB-mtl}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/tpcc_violinplot.png}
         \caption{\texttt{TPC-C}}
         \label{fig:TPC-C-mtl}
     \end{subfigure}
     }
        \caption{Estimation Error Residuals Distributions}
        \label{fig:violin-plots}
        \vspace{-10px}
\end{figure*}

\subsubsection{LearnedWMP Accuracy Performance}
\label{sec:learnedwmp-accuracy}
We report on LearnedWMP's accuracy performance in terms of RMSE. We also present the distribution of error residuals as violin plots for completeness.

\smallskip\noindent\textbf{RMSE}. Figure \ref{fig:model-training-rmse} reports the RMSEs of SingleWMP-based and Learned\-WMP-based models. SingleWMP-DBMS represents the state of practice in commercial DBMSs. LearnedWMP models and ML-based SingleWMP models significantly outperformed the SingleWMP-DBMS model. For the \texttt{TPC-DS}, SingleWMP-DBMS's RMSE was 1868. In comparison, LearnedWMP-DNN and LearnedWMP-Ridge, the two best ML models, had an RMSE of 169, which was a 90.95\% % reduction of the SingleWMP-DBMS estimation errors. SingleWMP-RF reduced SingleWMP-DBMS's estimation errors by 47.16\%. We see a similar pattern with \texttt{JOB} and \texttt{TCP-C} workloads, where, compared with the SingleWMP-DBMS method, all ML models produced more accurate estimations. In addition, figure \ref{fig:model-training-rmse} shows that the DNN and the XGBoost methods were highly accurate across all three datasets and with both SingleWMP and LearnedWMP approaches. Ridge methods were accurate with the LearnedWMP approach but had poor accuracy with the SingleWMP approach. From this observation, we deduce that linear algorithms, such as Ridge, may not be the best approach to model the memory demand of individual queries, represented using low-level database operations and their estimated cardinalities. 

\noindent \textit{On RMSE, ML-based methods --- LearnedWMP-based models and SingleWMP-based ML models --- were significantly more accurate than SingleWMP-DBMS method. Using heuristics, SingleWMP-DBMS couldn't accurately capture the complex interactions between database operators within a query plan and produced large estimation errors. In contrast, using ML, LearnedWMP-based, and SingleWMP-based ML models learned to estimate the memory requirements of complex database workloads more accurately.}

%\medskip\noindent\textbf{Interquartile Range (IQR) of the Estimates}. 
\smallskip\noindent\textbf{IQR and error distribution}. Figure \ref{fig:violin-plots} compares the violin plots of different models. The violins of the SingleWMP-DBMS are wider and far from zero. DBMS's estimations are skewed towards either underestimation or overestimation and span a larger region. In contrast, ML-based estimates are balanced between over and under-estimations and are not skewed. The violins of ML-based models span a smaller range than SingleWMP-DBMS's. For \texttt{TCP-DS}, LearnedWMP-DNN's violin is centered at zero and small. For the same dataset, SingleWMP-DBMS's violin is skewed toward underestimation and larger when compared to the IQR of LearnedWMP-DNN.  We see a similar pattern when comparing the violins of SingleWMP-DBMS models with the violins of other ML models. 

\noindent\textit{Using human-crafted rules, SingleWMP-DBMS's estimation errors are not distributed between overestimations and underestimations. These static rules skew the estimations toward one direction. In contrast, ML-based models learn from real-world workloads --- which include examples of both overestimation and underestimation --- and learn to compute memory predictions that are not skewed in one direction. For instance, the memory estimation errors of the DNN and XGboost methods for both SingleWMP-based and LearnedWMP-based models are smaller and balanced.}

%\subsection{LearnedWMP Training and Inference Cost}
\subsubsection{LearnedWMP Training and Inference Cost}

\begin{figure*}[t!]
     \centering
     \makebox[\linewidth][c]{%
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCDS-Training Time.png}
         \caption{\texttt{TPC-DS}}
         \label{fig:TPCDS-mtl}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/JOB-Training Time.png}
         \caption{\texttt{JOB}}
         \label{fig:JOB-mtl}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCC-Training Time.png}
         \caption{\texttt{TPC-C}}
         \label{fig:TPC-C-mtl}
     \end{subfigure}
     }
        \caption{ML model training latency}
        \label{fig:model-training-latency}
        \vspace{-10px}
\end{figure*}

\begin{figure*}[t!]
\makebox[\linewidth][c]{%
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCDS-Inference Time.png}
         \caption{\texttt{TPC-DS}}
         \label{fig:TPC-DS-mil}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/JOB-Inference Time.png}
         \caption{\texttt{JOB}}
         \label{fig:JOB-mil}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCC-Inference Time.png}
         \caption{\texttt{TPC-C}}
         \label{fig:TPC-C-mil}
     \end{subfigure}
     }
        \caption{ML model inference latency}
        \label{fig:model-inference-latency}
    \vspace{-10px}
\end{figure*}

\begin{figure*}
\makebox[\linewidth][c]{%
     \centering
     \begin{subfigure}[b]{0.33\textwidth}
         \centering         \includegraphics[width=\textwidth]{images/TPCDS-Model Size.png}
         \caption{\texttt{TPC-DS}}
         \label{fig:TPC-DS-ms}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/JOB-Model Size.png}
         \caption{\texttt{JOB}}
         \label{fig:JOB-ms}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/TPCC-Model Size.png}
         \caption{\texttt{TPC-C}}
         \label{fig:TPC-C-ms}
     \end{subfigure}
     }
        \caption{ML model size}
        \label{fig:model-size}
    \vspace{-10px}
\end{figure*}



Figure \ref{fig:model-training-latency} reports the training time of all models\footnote{Note that for this set of experiments, we do not consider LearnedWMP-DBMS as it is not an ML model and it doesn't have a training and an inference cost.}. For each benchmark dataset, LearnedWMP-based and SingleWMP-based methods use the same set of training queries as input. The singleWMP-based method uses individual training queries directly as input to the model. LearnedWMP batches the training queries into workloads, represents workloads as histograms, and uses the histograms as input to the models. Compared to SingleWMP-based models, the training of LearnedWMP-based models was significantly faster. For instance, with the \texttt{TPC-DS} dataset, SingleWMP-XGB was trained in 912.7 ms, whereas LearnedWMP-XGB was trained in 404 ms --- which is more than 2x faster. For all three benchmark datasets, we observe a similar trend: the training of a LearnedWMP-based model was faster than that of the equivalent SingleWMP-based model. The Ridge is the only algorithm that didn't demonstrate a significant difference in training time between the LearnedWMP and SingleWMP approaches. This is expected as Ridge is a linear algorithm that doesn't involve a sophisticated learning method.
%Across three datasets and both modeling approaches, in most cases, Ridge models trained in the fraction of time compared to other algorithms. 
Figure \ref{fig:model-inference-latency} compares the inference latency of SingleWMP-based and LearnedWMP-based models. The LearnedWMP-based models achieved between 3x and 10x acceleration compared to their equivalent SingleWMP-based models. As an example, for inference of \texttt{TPC-DS} workloads, LearnedWMP-DNN took 87.3 µs as compared to 870.5 µs needed by SingleWMP-DNN. Similarly, with \texttt{JOB}, LearnedWMP-XGB needed 313.3 µs for inference while SingleWMP-XGB took 1115.6 µs.

\noindent \textit{Accelerated training and inference performance of the LearnedWMP models can be attributed to our approach of formulating the training and inference task at the level of workloads, not at the level of individual queries. LearnedWMP-based models process batches of queries at the same time and, therefore, speed up the computation during both training and inference. In contrast, SingleWMP-based models require a longer time for training and inference as they work one query at a time.}

%\subsection{LearnedWMP Model Size}
\subsubsection{LearnedWMP Model Size}

%Smaller training set may not always produce smaller models. 
The model size largely depends on the learning algorithm and the feature space complexity of the training set. Figure \ref{fig:model-size} shows the size of LearnedWMP-based and SingleWMP-based models. LearnedWMP-based models were significantly smaller when compared with equivalent SingleWMP-based models. For example, when compared with SingleWMP-DNN, LearnedWMP-DNN is 59\% (\texttt{TPC-DS}), 72\% (\texttt{JOB}), and 97\% (\texttt{TPC-C}) smaller than SingleWMP-DNN. We see a similar pattern with XGBoost, RF, and DT when comparing their LearnedWMP-based models with equivalent SingleWMP-based models.
%, where the size of the LearnedWMP-based models were smaller than their SingleWMP-based counterparts.    

\noindent \textit{Batching training queries as workloads compress the information a LearnedWMP model needs to process during training. This compression helps the LearnedWMP approach produce smaller models as compared with models of the SingleWMP approach. Ridge is an exception to this observation. The size of a LearnedWMP-Ridge model is larger than its equivalent SingleWMP-Ridge model. This was expected as Ridge learns a set of coefficients, one for each input feature in the training dataset. In our training datasets, each LearnedWMP training example has more input features, one per query template, than the number of features in a SingleWMP training example. As a result, LearnedWMP-Ridge learns more coefficients during training and produces larger models.}

\subsubsection{Learning Query Templates}
As described in section \ref{subsection:learning-query-templates}, in the first phase of LearnedWMP, queries are assigned to templates based on their similarity in query plan characteristics and estimates, with the expectation that queries in the same template exhibit similar memory usage. We evaluated our method against four other approaches for learning query templates:
%assigns queries to templates in a way that queries with similar query plan characteristics and estimates are placed in the same groups. Our intuition is that queries in the same template have similar memory usage. We considered four additional methods for learning query templates and compared them with our method. Here's the list of methods we used in this comparison: 
\begin{enumerate}
    \item \textit{Query plan based (\textbf{query plan})}: Our proposed LearnedWMP model assigns queries to query templates by extracting features from the query plan and then employing a $k$-means clustering algorithm. Details can be found in section \ref{subsection:learning-query-templates}.
    \item \textit{Rule based (\textbf{rules})}: We create a set of rules, one per template, to classify a query statement into one of the pre-defined query templates. Subject matter experts, such as DBAs, may need to be involved in defining these rules \cite{zhou2020query}.
    \item \textit{Bag of Words based (\textbf{bag of words})}: %We extract unique keywords from the entire training query corpus to form a vocabulary. For each query expression, we obtain a feature vector that represents the number of times (count) each vocabulary word is found in the query. We apply the $k$-means clustering algorithm to assign the feature vectors into different query templates.
    We extract unique keywords from the entire training query corpus to build a vocabulary. Each query expression generates a feature vector representing the count of each vocabulary word in the query. The $k$-means clustering algorithm then assigns these feature vectors to different query templates.
    \item \textit{Text mining based (\textbf{text mining})}: This is a variation of the above bag of words approach. Bag of words indiscriminately extracts any unique keywords from the training query corpus. In contrast, in the text mining approach, the vocabulary includes only those keywords that are either database object names (e.g., a Table name) or SQL clauses (e.g., \texttt{group by}). Other keywords are ignored. After building a vocabulary, we apply similar steps to the bag of words approach to generate a feature vector for each query and then apply $k$-means clustering algorithm to assign them to templates.
    \item \textit{Word embeddings based (\textbf{word embeddings})}: %Word Embeddings are commonly used to overcome two limitations of the bag of words methods: a large number of keywords and failure to capture the proximity of keyword \cite{chollet2021deep}. %we construct a vocabulary of words from the training query corpus. Using the vocabulary, we generate a feature vector for each query expression. We then apply $k$-means clustering over these feature vectors to assign them to templates. 
    Word Embeddings address two limitations of bag-of-words methods: dealing with numerous keywords and capturing keyword proximity \cite{chollet2021deep}. Using word embeddings, With word embeddings, we construct a vocabulary from the training query corpus and generate a feature vector for each query expression. Applying $k$-means clustering assigns these feature vectors to templates.

\end{enumerate}

\noindent To evaluate the performance of the five alternative methods for learning templates, we used the LearnedWMP-XGB model with JOB workloads. We trained five LearnedWMP-XGB models, each using a different method for learning templates. Figure \ref{fig:templates} compares the accuracy of these five models. The model--- labeled query plan (ours) in the figure---that uses our original method for learning query templates outperformed the four alternatives. 

\noindent \textit{Compared with the alternatives, the LearnedWMP method uses features from the query plan. The query plans include estimates that are strong indicators of the resource usage of the queries. A prior research \cite{ganapathi2009predicting} made a similar observation. In contrast, the alternative methods extract features directly from the query expression, which does not provide insights into the query's memory usage. A major limitation of the rules-based method is that coming up with effective rules requires the knowledge of human experts, which can be both a difficult and a slow process.}

\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{images/JOB-Templates-RMSE.png}
  \caption{LearnedWMP's accuracy performance achieved by different methods for learning query templates.}
  %\Description{.}
  \label{fig:templates}
  \vspace{-10px}
\end{figure}

\begin{figure*}[t]
\makebox[\linewidth][c]{%

\begin{subfigure}[b]{.33\textwidth}
\centering
\includegraphics[width=.90\textwidth]{images/TPC-DS K Values.png}
\caption{\textbf{TPC-DS}}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.33\linewidth}
\centering
\includegraphics[width=.90\textwidth]{images/JOB K Values.png}
\caption{\textbf{JOB}}
\end{subfigure}%
\hfill
\begin{subfigure}[b]{.33\textwidth}
\centering
\includegraphics[width=.90\textwidth]{images/TPCC K Values.png}
\caption{\textbf{TPC-C}}
\end{subfigure}
}
\caption{MAPE at different template sizes with LearnedWMP XGBoost Model for the three evaluation datasets (a) TPC-DS, (b) JOB, and (c) TPC-C}
\label{fig:templatesizes}
\vspace*{-10px}
\end{figure*}


\subsubsection{Effect of the number of query templates}
\label{sec:effect-of-templates}
As described in section \ref{subsection:learning-query-templates}, LearnedWMP assigns queries into templates or clusters, such as queries with similar query plan characteristics in the same groups. This experiment aimed to assess the effects of the number of templates \texttt{(i.e., clusters)} on the LearnedWMP model's accuracy. In the experiment, we tested the performance of the LearnedWMP-XGB model on three datasets using 10 to 100 templates, comparing the model's performance across different template sizes. 

\noindent We used the Mean Absolute Percent Error (MAPE)~\cite{de2016mean} to evaluate and compare these models, each using a different number of templates.  %\footnote{\url{https://en.wikipedia.org/wiki/Mean_absolute_percentage_error}} .%, not RMSE that we used in the earlier experiments. 
 %With changes in the batch size, the error scale can significantly change. RMSE, which is impacted by the scale of the error value, is not suitable for comparing the relative performance of models trained with different batch sizes. 
 The scale of the error can vary significantly when changing the number of templates. MAPE  is unaffected by changes in the error scale when comparing models trained with different numbers of templates because it calculates a relative error. 
% MAPE, which computes a relative error and is not impacted by changes in the error scale, is more suitable for comparing models with different batch sizes.
We used equation (\ref{eqmse}) to compute the MAPE of the LearnedWMP-XGB model. 
\begin{align}
    MAPE = \frac{1}{N}\sum_{i=1}^N{\frac{|y_i-\hat{y_i}|}{y_i}} \times 100
    \label{eqmse}
\end{align}
We computed the relative estimation error between the actual and predicted memory utilization by dividing the absolute difference between them by the actual value and then averaged the relative estimation errors across all test workloads. The resulting average was multiplied by 100 to obtain the MAPE, ranging from 0 to 100 percent. Figure \ref{fig:batchsizes} shows the performance of LearnedWMP-XGB as a factor of the number of templates. 

\noindent Figure~\ref{fig:templatesizes} shows the performance of the LearnedWMP-XGB model for each template size for the three datasets; (a) \texttt{TPC-DS}, (b) \texttt{JOB}, and (c) \texttt{TPC-C}. In the case of the \texttt{TPC-DS} dataset, performance improved gradually with an increasing number of templates, with the best performance observed at 100 templates. However, for the \texttt{JOB} and \texttt{TPC-C} datasets, performance varied as the number of templates increased, with optimal performance achieved within the range of 20 to 40 templates. 

\noindent \textit{We argue that this correlation between the number of queries and the optimal number of templates can be attributed to the characteristics of each dataset. The larger \texttt{TPC-DS} dataset benefits from a greater diversity of queries \texttt{(93,000)} queries generated from \texttt{(99)} templates, which allows clustering with a higher number of templates. However, the smaller \texttt{JOB} and \texttt{TPC-C} datasets do not possess the same level of query variation, which explains why the best performance was achieved with a moderate number of templates (around 20 to 40).}


\subsubsection{Effect of the batch size parameter}
\label{sec:effect-of-batch-size}
The experiments we discussed so far used a constant workload batch size of 10. The batch size, $s$, is a tunable hyperparameter of the LearnedWMP model. We tried different workload batch sizes and compared their impact on the LearnedWMP model's accuracy. We used the \texttt{TPC-DS} dataset and the LearnedWMP-XGB model for this experiment. We used 12 values for the batch size: \texttt{[1, 2, 3, 5, 10, 15, 20, 25, 30, 35, 40, 45, 50]}. For each value, we created \texttt{TPC-DS} training and test workloads, which we used for training and evaluating a LearnedWMP-XGB model. We computed and used MAPE to compare the relative accuracy performance of these models. Figure \ref{fig:batchsizes} shows the performance of LearnedWMP-XGB as a factor of the batch size. We can see that with increasing batch size, the accuracy of the memory estimation improves. 

\noindent \textit{The improvement is more rapid initially, gradually slowing down, which is expected of any learning algorithm as it reaches the perfect prediction. For example, at batch size 2, the estimation error was 10.4\%. At batch size 10, the error was reduced to 3.8\%. We have seen a similar improvement in prediction accuracy with the remaining two experimental datasets. This observation substantiates our position that batch estimation of workload memory is more accurate than estimating one query's memory at a time.} Additionally, we compared the MAPE of the LearnedWMP model with batch size 1 with the SingleWMP model's MAPE. At batch size 1, LearnedWMP's MAPE is 10.2, whereas SingleWMP's MAPE is 3.6. 
%\noindent \textit{We can see that the SingleWMP model outperformed LearnedWMP batch 1. This is expected, as the SingleWMP model was trained directly with query plan features of each training query. These features provide strong signals to the memory usage of individual queries. In contrast, the LearnedWMP model maps each query in the input batch into query templates and then generates predictions. In this process, the predictive model doesn't learn from the individual features of each query; instead, it models the collective memory usage behavior of a batch of queries. When reducing an input workload to a batch of 1 query, the LearnedWMP model used weaker signals than SingleWMP to generate prediction at the level of single queries. However, as we have seen in \ref{sec:learnedwmp-accuracy}, LearnedWMP generates more accurate predictions than SingleWMP when generating predictions for batches of queries.}
\noindent \textit{The SingleWMP model outperformed the LearnedWMP batch 1 model, which was expected since SingleWMP was directly trained with query plan features, providing strong signals for individual query memory usage. In contrast, the LearnedWMP model mapped queries into templates and generated predictions based on collective memory usage, lacking the ability to learn from individual query features. While LearnedWMP had weaker signals for single query predictions, it demonstrated higher accuracy than SingleWMP when generating predictions for query batches. However, as we have seen in \ref{sec:learnedwmp-accuracy}, LearnedWMP generates more accurate predictions than SingleWMP when generating predictions for batches of queries.}
%%%%%HERE
%\subsubsection{Effect of different featurization techniques}We assessed various feature encoding methods that followed the set-based query representation approaches described in \cite{kipf2018learned} and \cite{negi2023robust}. Our approach involved combining fundamental relational details and query features (such as join keys, table names, and predicates) into a one-hot encoding, which was then used for predicting memory estimates. In our evaluation, we also leverage these features to classify queries into templates, effectively replacing the clustering phase in our methodology.

%We argue that this is correlated to the number of queries in each dataset; \texttt{TPC-DS} contains 93000 queries generated from many query templates (e.g., 99 templates). However, the \texttt{JOB} and \texttt{TPC-C} were smaller datasets of 2300 and 3958 queries, respectively. 

%We generated 93000 queries for TPC-DS, 2300 queries for JOB, and 3958 queries for TPC-C. For each benchmark
\begin{comment}
\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{images/plots/job_cluster_result.png}
  \caption{TPC-DS RSME at different template sizes with LearnedWMP XGBoost Model.}
  %\Description{.}
  \label{fig:templatesizes}
  \vspace{-10px}
\end{figure}

\begin{figure*}
  \begin{minipage}[t]{0.32\linewidth}
    \includegraphics[width=\textwidth]{images/plots/JOB K Values.png}
    \caption{Impact of training data (\#triplets per entity).}
    \label{fig:varying_triplets}
  \end{minipage}
  \hspace{1mm}
  \begin{minipage}[t]{0.32\linewidth}
    \includegraphics[width=\textwidth]{images/plots/TPCC K Values.png}
    \caption{Impact of compression on Recall@K.}
    \label{fig:recall_pq}
  \end{minipage}
  \hspace{1mm}
  \begin{minipage}[t]{0.32\linewidth}
    \includegraphics[width=\textwidth]{images/plots/TPC-DS K Values.png}
    \caption{Comparing the performance of Product Quantization and PCA.}
    \label{fig:pca_plots}
  \end{minipage}
   \caption{RSME at different template sizes with LearnedWMP XGBoost Model.}
\end{figure*}
\end{comment}




==> introduction.tex <==
%\section{INTRODUCTION}
%\label{sec:intrhttps://www.overleaf.com/project/61cbb313131d4106e11abaa2o}
%\smallskip\noindent\textbf{Motivation}. 
%For decision making tasks in databases, such as admission control, workload management, and capacity planning, and for the successful operation of queries, it is crucial to know the resource usage of the queries \cite{ganapathi2009predicting}. 
Estimating resource usage of database queries is critical to many database operations and decision-making tasks, such as admission control, workload management, and capacity planning~\cite{ganapathi2009predicting}. Working memory is a region of the system memory where DBMS may perform different in-memory operations, such as sort and aggregation while executing queries. 
Using a limited system memory, DBMS can execute a finite number of in-memory operations, thus queries, simultaneously. Inaccurate estimations of working memory demands of the queries cause the DBMS to either under or over-commit the memory, which prevents the DBMS from achieving optimal query performance - faster query execution and higher throughput, and may also lead to query failures. For high query performance, the DBMS needs accurate working memory estimations of the queries before admitting them for execution.  

%\stitle{Workload Memory Prediction} Given a batch of queries, as workload, this task aims to predict the amount of working memory needed to execute this workload on a DBMS. Predicting memory demand depends on historical queries and other factors.To do this, we use the LearnedWMP model, which predicts memory usage based on historical queries and other factors. This model can be used to address the admission control scenario mentioned in the review. The DBMS workload management component can create a batch of all committed queries and incoming queries from the queue. The batch can be sent to the LearnedWMP pipeline to estimate total working memory usage. The workload manager can obtain the memory estimate for incoming queries by subtracting memory already allocated for committed queries from the estimate. Prediction at the level of workloads can provide multiple benefits. First, it helps DBMS’s workload manager make more accurate admission control decisions for incoming queries. Instead of the state-of-the-art practice of looking into each query separately and estimating its working memory usage, the workload manager can form a batch of queries and generate its collective memory usage. If the collective memory usage is below the threshold of available memory, the DBMS can commit the workload. LearnedWMP can handle multiple workload admission scenarios: (1) the workload consists of all non-committed queries, and (2) the workload consists of committed and uncommitted queries.  (1) An example scenario of the first use case is assisting a DBA to schedule a workload. The DBA can send the workload batch to the LearnedWMP model and get a prediction on its collective memory usage. Based on the prediction, the DBA can decide whether to schedule the workload. (2) When a new query or a set of queries arrive at the DBMS, the workload manager can form a workload by including all the already committed queries and the incoming queries and run by the LearnedWMP model to get a prediction of the collective working memory usage of the entire workload. By subtracting the allocated memory for the already committed queries, the DBMS can get the estimated memory usage of the incoming queries. The workload manager can commit these incoming queries if this estimate is below the available system memory. 




%In a contemporary DBMS, the query optimizer’s cost model derives cardinality estimates based on simplified assumptions that distinct column values are uniformly distributed for join cardinality estimation and that, without advanced statistics, columns are independent of each other. Both the uniformity and independence assumptions of the data are often wrong and eventually lead to inaccurate memory estimations \cite{leis2017cardinality, leis2015good}. In addition, the DBMS derives estimations for each query separately \cite{ganapathi2009predicting}, without exploiting the insight that concurrent queries execute operations that often stress certain resource utilization, e.g., memory, on the system. For illustration, when a DBMS processes two concurrent queries with each including a \texttt{group by} operation, their collective memory demand can be higher than executing each separately. When the collective memory requirement exceeds the available system memory, some of the queries take longer to finish, which increases query execution time and decreases DBMS's throughput. In the state of the practice, human experts define the features and the rules for calculating runtime metrics of the queries \cite{marcus2019plan}. Relying on human experts is expensive. Additionally, these estimation rules do not generalize well to unseen workloads and to new operational environments of the DBMS.

\smallskip\noindent\textbf{{\color{red} The state of the practice \& limitations}}. In contemporary DBMS, the query optimizer's cost model faces several limitations. Firstly, it tends to derive estimations for each query independently, missing the opportunity to leverage insights from batch queries that collectively stress specific resource utilization, such as memory \cite{ganapathi2009predicting}. For example, processing two queries with a \texttt{group by} operation can exceed the memory demand of executing each query separately. If this collective memory requirement surpasses available system memory, it can lead to increased query execution times, decreasing the DBMS's throughput. In current practice, Human experts traditionally define features and rules for calculating runtime metrics of queries, but this is an expensive and non-generalizable approach \cite{marcus2019plan}.  %For instance, when processing two queries with a \texttt{group by} operation, their combined memory demand can exceed that of executing each query separately.When dealing with single queries, there is overhead associated with memory allocation, deallocation, and management for each query. Batching queries mitigates this overhead by enabling the system to allocate memory more efficiently for multiple queries at once.Predicting memory requirements for a batch of queries provides a more accurate estimate of the total memory needed for a single query execution. This helps avoid over-allocation or under-allocation of memory resources, leading to improved stability and performance. 
To our knowledge, there is currently no practical engine or optimizer capable of predicting memory requirements for a batch of queries. Predicting memory needs for a batch of queries provides a more accurate estimate of the total memory required for executing a single query, aiding in preventing over-allocation or under-allocation of memory resources, and contributing to enhanced system stability and performance. Another limitation of the optimizer's cost model lies in its reliance on simplified assumptions, specifically in the cardinality estimation. These assumptions involve expecting a uniform distribution of distinct column values for join cardinality estimation and assuming that, in the absence of advanced statistics, columns are independent. %Unfortunately, these assumptions frequently turn out to be inaccurate, resulting in imprecise memory estimations. 
It is worth mentioning that cardinality estimation is a distinct task from working memory estimation. However, the aforementioned assumptions often lead to inaccuracies, contributing to imprecise memory estimations \cite{leis2017cardinality, leis2015good}.

%\cite{leis2017cardinality, leis2015good} 
\smallskip\noindent\textbf{The state of the art \& limitations}. In recent years, many researchers proposed deep learning-based methods for addressing query optimization problems \cite{han2021cardinality, hilprecht2019deepdb}, especially for cardinality estimation \cite{yang2020neurocard, liu2015cardinality, hilprecht2019deepdb, kipf2018learned, hasan2020deep}, which closely relates to memory usage estimation. These methods are promising as they can learn hidden patterns in the data and understand relationships between interdependent variables. Nonetheless, there is currently insufficient evidence that these methods are suitable for enterprise-grade DBMS instances and their applicability to the task of predicting working memory\cite{han2021cardinality}. This is because they are usually evaluated with simplified benchmark datasets that do not represent the complex characteristics of enterprise data \cite{han2021cardinality}. These methods also require complex hyper-parameter tuning that can limit reproducibility and interoperability. Readers are encouraged to refer to \cite{kim2022learned} for a detailed analysis of learned cardinality estimators for single queries and their limitations. Deep learning models for single query memory estimation may not generalize effectively to workload memory prediction.

\smallskip\noindent\textbf{Our approach}. We propose a novel approach for estimating resource usage of a batch of database queries, a {\em workload}. Our approach is a departure from the existing approach of estimating the resource usage of each query separately. We exploit the observation that DBMS executes queries concurrently and that concurrent queries often have competitive resource demands. By modeling the resource demand of concurrent queries, we expect to achieve higher accuracy in estimating resources. Also, we expect our approach will reduce the development and maintenance costs of the DBMS's resource estimator and speed up the computation of resource estimations. As an embodiment of our idea, we initially focused on estimating the working memory of database workloads. We design a \underline{Learned} \underline{W}orkload \underline{M}emory \underline{P}rediction (LearnedWMP) model in three steps. {\em First}, we use an intuition that queries with similar plan characteristics and estimated cardinalities have similar memory demand. Based on this intuition, we use historical queries to learn {\em query templates} that serve as groups for queries with similar memory demands. {\em Second}, we randomly divide training queries into fixed-size training workloads and represent each workload as a {\em histogram} - {\em a distribution of query templates}. A histogram-based representation allows capturing the underlying statistical distribution of the queries by grouping them into bins or templates. Histograms have been used in different domains to aggregate multiple observations and obtain approximate data distributions \cite{Koloniari}. To simplify the experiment setup, the current design of LearnedWMP uses fixed-length workloads. However, the design can easily be extended to work with variable-length workloads. In {\em the final step}, using training workloads and their historical collective actual memory usage, we train a regression model that learns to estimate the working memory usage of an unseen workload based on the distribution of query templates. As the model learns from diverse training workloads, its accuracy at estimating the working memory of workloads will improve with time. 

\stitle{Summary of Experimental Results.} 
We conducted extensive experiments demonstrating that LearnedWMP significantly reduced memory estimation errors in comparison to the state-of-the-art practice, achieving a remarkable 47.6\% improvement. Our experiments are conducted over three major database transactional and analytical benchmarks that are used to train and evaluate our model. LearnedWMP accepts as input a workload and returns the workload’s estimated working memory demand for the workload. Given that there are no existing libraries or methods for this novel problem, we develop and evaluate different variations of LearnedWMP and compare them to alternative single-query ML models. Our findings indicate that, during training and inferencing, the LearnedWMP models were 3x to 10x faster compared to alternative ML models.; also, LearnedWMP models were at least 50\% smaller in most cases. Furthermore, our study delved into the performance and impact assessment of different components and parameters within the model. These included various learning models, workload sizes, numbers of query templates, and techniques for learning query templates (such as query plan-based and rule-based approaches). %Overall, the results show the advantages of the LearnedWMP approach, highlighting its potential to enhance query performance with significantly broader implications.

\stitle{Contributions}. We summarize our key contributions as follows: 
\begin{enumerate}
    \item We introduce a novel approach to {\em predicting memory usage of database workloads}. To the best of our knowledge, this is the first attempt to predict a workload's memory demand using machine learning techniques. 
    \item We formulate the problem of workload memory prediction as {\em a distribution regression problem}, which learns a regressor function from workloads represented as distributions of query templates. We use machine learning techniques to learn the regressor without relying on the hand-crafted query-level or operator-level features. 
    \item We propose LearnedWMP, a novel prediction model that can estimate the working memory demand of a batch of SQL queries in a workload at once. This is a departure from the state of the practice and the state-of-the-art methods, which estimate the memory demand of each query separately.
    \item We devise unsupervised machine learning methods to group queries of similar memory needs to significantly reduce the computational overhead of workload memory usage estimation.
    \item We extensively evaluate our LearnedWMP model employing three database benchmarks --- two analytical and one transactional. Our model significantly reduced the memory estimation errors of DBMS by at least 47.16\%. These experimental results prove the merit of our proposed technique in workload-based query processing and resource estimation.
\end{enumerate}
%\smallskip\noindent\textbf
\stitle{DBMS integration \& broader impact}. A DBMS vendor can pre-train a LearnedWMP model using sample training workloads and ship the model into the DBMS product. With the deployment of the DBMS on an operational site, the pre-trained LearnedWMP model can immediately generate memory estimations, which may not be highly accurate initially. DBMS can collect training workloads from its operational environment and use them to re-train the LearnedWMP model to improve the model's estimation accuracy. Major DBMS products \footnote{\url{https://www.ibm.com/docs/en/db2/11.5?topic=content-in-database-machine-learning}}\footnote{\url{https://learn.microsoft.com/en-us/sql/machine-learning/}}\footnote{\url{https://www.oracle.com/ca-en/artificial-intelligence/database-machine-learning/}} now include ML infrastructure, which they can use for hosting, training, and serving the LearnedWMP model in the database.

\smallskip\noindent\textbf{Paper organization}. The rest of the paper is organized as follows. Section \ref{sec:problem} introduces key terminology, notations, and the problem formally. Section \ref{sec:methodology} provides an overview of LearnedWMP, including details of the training and inference stages. Section \ref{sec:evaluation} presents an experimental evaluation of LearnedWMP. Section \ref{sec:related} reviews the related work. Section \ref{sec:conclusions} concludes the paper. 

%In this work we try to address and improve the memory prediction using histogram data, 

 %deploying modern data-driven applications and online services. 
%\marin{need to rewrite the remainder of this paragraph, the text is too repetitive; develop it around the idea that resource policies are based on workload estimation and that the current estimations; give some examples of resource management tasks where estimations are used; Need to motivate why resource consumption estimations are strong motivator of this work.} 


%Handling this complex task requires the DBAs to gain a deeper understanding of the characteristics of the query workload. 
 %So, coming up with tuned database configuration to achieve better query performance is not an one-time thing. It's an ongoing task requiring high degree of human efforts.

%In this work we try to address the following research problem: \marin{I would not use this question, takes the reader in a different direction} ``for a given workload waiting to be executed immediately, should the system accept this workload or not.'' This is an important decision the DBMS  needs to make based on the demand that the workload will bring to the system. \\
 
%\textit{\textcolor{red}{The following para talks about a brief discussion on past works and their disadvantages followed by research gap}}\\
 %\\
 %\par \marin{ if the previous paragraph was about explaining why estimation of workloads and resource  is important, focus in this paragraph on the limitations of current approaches and why another estimation method is needed ; not sure if you need a complete related work; need to check VLDB if the typical paper requires a "related work" section}Often the database admits wrong workloads based on incorrect resource demand estimates.  \\
%\\
%\textit{\textcolor{red}{What we are doing and why (Motivation and Justification), brief discussion on methodology and the advantage of the proposed method}}\\
%\marin{you just need to provide the high level description of the work and why justify us to hypothesize that it will work; motivation was probably covered earlier}

%\textcolor{red}{Not clear --The approach of aggregating data and representing in the form  of histogram is useful in this era of big data, since histogram can not only save storage space but also represents types of workloads from a global viewpoint.} 
% \par The above research attempts can be broadly put into 2 categories: (a) predicting the future workloads and (b) predicting the system performance. For the first scenario, the predictive models forecast the volume of workload incoming to a  system. For the second scenario, the model predicts system performance under various situations. For example, how will the system perform if the volume of workload doubles or how will the system perform if certain hardware resource (e.g. memory) is increased by a certain amount? 
 
%\textit{\textcolor{red}{This para presents a brief literature survey of past works on database problems solved by ML approaches and how our approach in a bird's eye view.}}\\
 
%\marin{shouldn't the next para be part of a related work section?}
  


==> methodology.tex <==
%\section{The L\MakeLowercase{earned}WMP Model}
%\section{L\MakeLowercase{earned}WMP S\MakeLowercase{ystem}}
%\label{sec:methodology}

%The \textsc{LearnedWMP} model has two stages: training and inference. The training stage executes a machine learning training pipeline, a predefined sequence of steps, to construct a learnedWMP model. The inferencing stage uses the LearnedWMP model, generated from the training stage, to compute memory estimates for unseen workloads. Figure 1 shows an schematic overview of both stages of LearnedWMP. Here we briefly describe these stages, which we'll detail later in this section.

%The \model model has two stages: {\em training} and {\em inference}. The training stage uses a machine learning pipeline and a training dataset to build a \model model. The inference stage uses the trained \model model to predict memory usage for unseen workloads. Figure \ref{fig:ml-pipeline} shows an overview of the \model workflow. In this section, we first briefly describe the steps of this workflow and then discuss the technical details of each step. 
LearnedWMP comprises two stages: training and inference. The training stage employs a machine learning pipeline and dataset to build the model, while the inference stage utilizes the trained model to predict memory usage for unseen workloads. Figure \ref{fig:ml-pipeline} offers an overview of the workflow, and we subsequently outline and delve into the technical details of each step.

\begin{figure*}
  \includegraphics[width=\textwidth]{images/LearnedWMP Workflow 8.png}
  \caption{Overview of the \model model. Left: Users send queries to a DBMS; the DBMS processes and sends responses to the queries. Right-upper: the training steps of the \model model. Right-bottom: the steps of the inference stage.}
  %\Description{.}
  \label{fig:ml-pipeline}
  \vspace{-10px}
\end{figure*}

\subsection{Overview of the \model 's pipeline}
%\smallskip\noindent\textbf{Training stage}. 
\stitle{Users and the database} The top left section of Figure \ref{fig:ml-pipeline} illustrates user-database interaction, with the database interacting with two \model stages. The users and applications send SQL queries to the database. To calculate the memory utilization of a workload, we sum the highest memory usage for queries in that workload. The \model training pipeline (right section of Figure \ref{fig:ml-pipeline}) periodically retrains the model using the latest query log dump.

\stitle{Training stage} In Figure \ref{fig:ml-pipeline} (top), \texttt{TR1} through \texttt{TR6} are the steps of the training pipeline. Training begins with a set of training queries, $\mathcal{Q}_{train}$, collected from a dump of the DBMS query log. At \texttt{TR1}, from $\mathcal{Q}_{train}$, the pipeline extracts training queries, their final execution plans, and the actual highest working memory usage from the past execution. At \texttt{TR2}, from the query plans, the pipeline generates a set of $m$ features to represent the training queries as a $|\mathcal{Q}_{train}| \times m$ feature matrix. 
%Here, $|TQ|$ is the number of training queries and $m$ is the number of generated query plan features to represent each training query. 
At \texttt{TR3}, the pipeline learns $\mathcal{T}$, a set of $k$ query templates, from the query feature matrix. the value of $k$ can be determined experimentally (cf. section \ref{sec:methodology-training}). At \texttt{TR4}, the pipeline equally divides the training queries of $\mathcal{Q}_{train}$ into a set of $n$ workloads, $\mathcal{W}$  = $|\mathcal{Q}_{train}|/s$. Each workload contains $s$, a constant, queries. We found a value of $s$ experimentally (cf. subsection \ref{sec:sensitivity}). At \texttt{TR5}, the pipeline generates a workload histogram $\mathcal{H}$ for each training workload $w$ = $(\mathcal{Q}, y)$ in $\mathcal{W}$.  $\mathcal{H}$ represents the distribution of queries of $\mathcal{Q}$ among $k$ query templates of $\mathcal{T}$. In addition, the collective actual highest memory utilization $y$ of the workload $w$ is computed by summing up the working memory utilization of each query $q_i \in \mathcal{Q}$. Each ($\mathcal{H}$, $y$) pair represents a supervised training example for training a regression model. At \texttt{TR6}, the model receives as input a collection of training examples of the form ($\mathcal{H}$, $y$). From these examples, the model learns a regression function $\hat{f}(\mathcal{H})$ to map an input histogram $\mathcal{H}$ to its working memory demand, $y$. At the end of \texttt{TR6}, the training pipeline produces a trained \model model.
%\smallskip\noindent\textbf{Inference stage}. 

\stitle{Inference stage} In Figure \ref{fig:ml-pipeline} (bottom), \texttt{IN1} through \texttt{IN5} are the steps of the  \model inference pipeline, which generates estimated memory usage of an unseen workload $w$, consisting of $\mathcal{Q}$ queries. Step \texttt{IN1} collects the query plans of the queries $\mathcal{Q}$ in $w$; step \texttt{IN2} generates the feature vectors for these plans. Step \texttt{IN3} assigns each query $q_i \in \mathcal{Q}$ to a template $t_i \in \mathcal{T}$, from which \texttt{IN4} constructs a workload histogram $\mathcal{H}$. The final step, \texttt{IN5}, uses the histogram $\mathcal{H}$ as input to the \model model and predicts the memory usage $\hat{y}$ of the workload, $w$.

%\subsection{Training Stage of the L\MakeLowercase{earned}WMP Model}
\subsection{L\MakeLowercase{earned}WMP: Training Stage}
\label{sec:methodology-training}

We train the \model model in six steps, \texttt{TR1} through \texttt{TR6}, which we can semantically group in three {\em phases} (see figure 1). The first phase uses historical queries from a DBMS's query log to learn a set of {\em query templates}. The second phase prepares the {\em training dataset}, a collection of training examples, for the learning algorithm. The third phase uses the {\em training dataset} to train a {\em regression model}, which can predict the memory usage of an input workload.

\subsubsection{Phase 1: Learning Query Templates} 
\label{subsection:learning-query-templates}
We assign queries to templates based on the intuition that queries with similar query-plan characteristics and cardinality estimates have similar execution-time memory usage. In each workload, by grouping similar queries in the same templates or clusters, we expect to model more efficiently the memory requirements of the queries and speed up the computation of training and inference stages. We are not looking for an optimal template assignment for each query, which will require computation of operator-level features, increase computation overhead, and outweigh the acceleration we hope to gain from compressing queries into templates. Also, estimating the cost of individual queries is a separate research problem \cite{ganapathi2009predicting, li2012robust} that we are not addressing in our current research. Instead, we rely on a best-effort algorithmic principle for assigning each query to a template. The template assignment needs to be just good enough, not highly accurate. This allows designing simple but efficient methods for assigning queries to templates that neither jeopardizes the runtime cost nor the machine learning approach. This is not an algorithmic simplification but rather an algorithmic design choice.

\noindent To assign queries to templates we use standard $k$-means clustering algorithm \cite{macqueen1967classification}. Algorithm \ref{algo:kmeans} describes the steps of \textsc{GetTemplates} function that uses training queries of $\mathcal{Q}_{train}$ to learn a set of $k$ query templates, $\mathcal{T}$. For each query in $\mathcal{Q}_{train}$, \textsc{GetTemplates()} first extracts the query plan (line 5). A query plan is a tree-like structure where each node corresponds to a database operator. The plan's execution begins at the leaf nodes and completes at the root node. The output of the root is the result of executing the entire query. Each node has an input and an output. When applicable, a node includes statistics, such as estimated pre-cardinality and post-cardinality of the operator. For each operator type in a query plan, \textsc{GetTemplates()} counts its frequency and aggregate cardinalities of all its instances. The frequency count and aggregated cardinality of each operator type are retrieved (line 6) and used to represent the {\em query features}. Finally, the $k$-means algorithm \cite{macqueen1967classification} uses these query feature vectors to learn $k$ clusters, each one representing a query template $t_i \in \mathcal{T}$ (line 8). We use the elbow method \cite{raschka2019python} to tune the value of $k$. Figure \ref{fig:feature-extraction} provides an illustrative example query, where its associated query plan tree (below) has five unique operators: \texttt{TBSCAN}, \texttt{HSJOIN}, \texttt{INDEX SCAN}, \texttt{SORT}, and \texttt{GROUP BY}. Since each operator type provides a (count, cardinality) pair of features (\# of operators, total cardinality), this sample query plan has 10 features - 2 features for each of the 5 operators. \textsc{GetTemplates()} encodes these features in a 1-$d$ vector as follows: 
\noindent \texttt{[4, 139532.48, 3, 50224.6, 1, 3201, 1, 134179, 1, 48873.6]}.
%The method consists of plotting the explained variation as a function of the number of clusters and picking the elbow of the curve as the number of clusters to use.
%[t]
%\begin{figure}
\begin{algorithm}[H]
 \caption{Learning query templates with $k$-means clustering}
 \label{algo:kmeans}
    \begin{algorithmic}[1]
  \State $\mathcal{Q} {train} \leftarrow \{q_1,\ q_2,...,\ q_n\}$ \Comment{$\mathcal{Q}_{train}$ is a set of historical training queries collected from a DBMS.} 
     \Function{GetTemplates}{$\mathcal{Q}_{train}$}
   %    \FunctionCall{GetTemplates}{$\mathcal{Q}_{train}$}
          \State $Array\ Z \leftarrow [][]$ \Comment{feature matrix for $\mathcal{Q}_{train}$}
         \For{$q_i \in\ \mathcal{Q}_{train}$}
         \State $plan_i$ = getQueryPlan($q_i$)
         \State $features_i$ = getFeatures($plan_i$)
        \State Z.insert($features_i$)
         \EndFor
        \State $\mathcal{T} \leftarrow kmeans(Z, k)$ \Comment{learns templates using kmeans}
        \Return $\mathcal{T}$ \Comment{\textit{k} learned query templates}
    \EndFunction
 \end{algorithmic}
\end{algorithm}
%\end{figure}

\subsubsection{Phase 2: Constructing Histograms from Workloads}
In this phase, \model performs two tasks: ({\em i}) partitions training queries of $\mathcal{Q}_{train}$ into a set workloads, $\mathcal{W}$ and ({\em ii}) from each training workload, $w_i \in \mathcal{W}$, constructs a histogram that represents the distribution of its queries among the query templates set $\mathcal{T}$. Histograms have played a significant role in estimating query plans cost \cite{bruno2002exploiting}. \model randomly divides training queries from $\mathcal{Q}_{train}$ into $m$ training workloads, where $m = |\mathcal{Q}_{train}| / s$ with $s$ being a constant number of training queries per workload. The value for $s$ depends on the application domain and can be empirically found (cf. subsection \ref{sec:sensitivity}). As defined in \textit{definition 2.2}, each training workload, $w_i$, is a tuple $(\mathcal{Q}, y)$, where $\mathcal{Q}$ is a collection of queries and $y$ is their collective memory usage from the past execution.\\
Algorithm \ref{algo-kmeans-Templatizing} describes the steps of phase 2. It takes as input a training workload, $w$, and a set of query templates, $\mathcal{T}$, which were learned in phase 1. In \texttt{lines 6-7}, for each query $q_i \in \mathcal{Q}$, the algorithm extracts the query execution plan and the features from the plan. Since phase 1 already computed these features, \texttt{line 7} reuses the values from the previous computation. Using these features, \texttt{line 8} looks up the query template, $t_j \in \mathcal{T}$, for $q_i$. After assigning each query, $q_i \in \mathcal{Q}$, to a template, the algorithm counts the number of queries in $\mathcal{Q}$ in each template, $t_j \in \mathcal{T}$ (\texttt{line 10}) and stores the counts in a histogram, a 1-d count vector, $\mathcal{H} = [c_1, ...,c_{k=|\mathcal{T}|}]$. The length of $\mathcal{H}$ is $k$, corresponding to the number of query templates in $\mathcal{T}$. Each count $c_j \in \mathcal{H}$ is the number of queries in $w$ that are associated with the query template $t_j \in \mathcal{T}$. These counts add up to $s=|\mathcal{Q}|$, the workload batch size:
\begin{equation}
\sum_{j=1}^{k=|\mathcal{T}|} c_j = s   
\end{equation}
%

\noindent The histogram $\mathcal{H}$ is the distribution of queries in workload $w$ among the query templates set $\mathcal{T}$. The histogram will be sparse with many zeros as a workload is not expected to contain queries that belong to each query template of $\mathcal{T}$. At the final step (\texttt{line 11)}, the algorithm returns a pair ($\mathcal{H},y$), where $y$ is the collective memory usage of all $q \in \mathcal{Q}$. ($\mathcal{H},y$) becomes a labeled example for training a supervised machine learning model in Phase 3.

\begin{figure}[t]
  %\includegraphics[width=0.45\textwidth]{images/plots/query2vec2.png}
    \includegraphics[width=0.45\textwidth]{images/queryplan8.png}
  \caption{Extracting query features from a query. An example query (top) is executed by the query plan (left), leading to the extraction of the query features (right). The query features are used to learn a set of query templates $\mathcal{T}$, of size $k$.}
  \label{fig:feature-extraction}
  \vspace{-10px}
\end{figure}

\noindent Figure \ref{fig:binning} shows an example of constructing a histogram $\mathcal{H}$ of 4 bins, $k=|\mathcal{T}|=4$. The example uses an input workload, $w$, with 9 queries, $s=|\mathcal{Q}|=9$. $3$ of $4$ histogram bins are populated with nonzero values. The remaining bin has a zero value as its corresponding query template has no queries in $w$. The histogram vector is \texttt{[3, 4, 0, 2]}. The value of $y$ is the total actual memory usage of the historical memory usage of all 9 queries in $w$. Let's assume $y$ = \textit{125} MB. The output pair for this example workload is (\texttt{[3, 4, 0, 2]}, \textit{125}). 

\subsubsection{Phase 3: Training a Distribution Regression Deep Learning Model}
%\subsubsection{Phase 3: Training a Deep Learning Model for Distribution Regression}
In this phase, we train a regression model for predicting workload memory usage. The trained model takes an input workload, represented as a histogram of query templates, and computes the workload's memory usage. We explored several machine learning and deep learning techniques to train the model. In this subsection, we will present the design and implementation of a deep learning (DL) model for our regression model. Section \ref{sec:other-ml-methods} describes the other machine learning algorithms we explored for the model training. DL recently had several algorithmic breakthroughs and has been highly successful with many learning tasks over unstructured data. For example, DL models for image recognition and language translation are now highly accurate \cite{shwartz2021tabular}. Additionally, DL can be useful in learning a non-linear mapping function between input and output without requiring low-level feature engineering. In our case, we have dual complexities: the input is a complex distribution of query templates, and there is a complex relationship between the distribution of query templates and its collective memory demand. We wanted to explore the effectiveness of deep learning for the problem. 

\noindent\textbf{Multilayer Perceptron (MLP) Model}. Various deep learning networks have been developed for unstructured data, such as convolution neural network (CNN) \cite{lecun1989backpropagation} for images; recurrent neural network (RNN) \cite{salehinejad2017recent} and transformers \cite{vaswani2017attention} for sequential data, and graph neural networks (GNN) for graphs \cite{murphy2022probabilistic}. Unstructured data often has variable-length input vectors with individual elements lacking meaning in isolation \cite{murphy2022probabilistic}. However, in our case, the input vector for each workload is structured and has a fixed length corresponding to the number of query templates. Each vector element represents the workload queries of a specific template. 
Since we want to learn a regression function from fixed-length input vectors, the multilayer perceptron (MLP) is a suitable choice for learning a regression function from fixed-length input vectors due to its assumption of fixed input dimension and flexibility in architecture~\cite{murphy2022probabilistic, subasi2007eeg}. %MLP offers the benefits of stochastic problem-solving, fast operation, ease of implementation, and smaller training set requirements~\cite{subasi2007eeg}. %MLP architecture consists of input, hidden, and output layers, with the hidden layers transmitting and processing input information. Choosing an appropriate number of hidden layer neurons is crucial to avoid overfitting and lack of generalization, but there is no analytical method for determining the ideal number. Therefore, it is only found by trial and error \cite{haykin2009neural}. MLP architecture consists of input, hidden, and output layers where hidden layers process input information, and the optimal number of hidden layer neurons is determined through trial and error since there is no analytical method to precisely determine the ideal number, which is crucial to prevent overfitting and ensure generalization \cite{haykin2009neural}. In our case, from $n$ training examples $(\mathcal{H}_1, y_1), (\mathcal{H}_2, y_2),\ldots,(\mathcal{H}_n, y_n)$, a MLP model learns a function $f(\cdot): R^k \rightarrow R^o$, where $k$ is the number of dimensions for input $\mathcal{H} = [c_1, ...,c_{k=|\mathcal{T}|}]$ and $R^o$ is the scalar output $y$. 
MLP architecture consists of input, hidden, and output layers, and the optimal number of hidden layer neurons is determined through trial and error since there is no analytical method to precisely determine the ideal number crucial to prevent overfitting and ensure generalization \cite{haykin2009neural}.
In our case, from $n$ training examples $(\mathcal{H}_1, y_1), (\mathcal{H}_2, y_2),\ldots,(\mathcal{H}_n, y_n)$, a MLP model learns a function $f(\cdot): R^k \rightarrow R^o$, where $k$ is the number of dimensions for input $\mathcal{H} = [c_1, ...,c_{k=|\mathcal{T}|}]$ and $R^o$ is the scalar output $y$.

%Algorithm \ref{alg:trainmodel} presents the steps of a function \textsc{TrainModel()} that trains the MLP model (i.e., updating the model weights until they convergence).
\begin{comment}
    

\noindent\textbf{Multilayer perceptron (MLP) model}. Many DL networks exist for learning from unstructured data, such as images and text. For example, convolution neural network (CNN) \cite{lecun1989backpropagation} is suitable for working with images; recurrent neural network (RNN) \cite{salehinejad2017recent} and transformers \cite{vaswani2017attention} work with sequential data; graph neural networks (GNN) are available for graphs \cite{murphy2022probabilistic}. With unstructured data, the dimension of the input vector has a variable length, and each element in the vector usually has no meaning in isolation \cite{murphy2022probabilistic}. In our case, the input vector for each workload is structured and has a fixed length corresponding to the number of query templates. Each element of the vector represents the number of workload queries belonging to a specific template. Since we want to learn a regression function from fixed length input vectors, multilayer perceptron (MLP) is a good place to begin with as it assumes the input data has a fixed dimension \cite{murphy2022probabilistic}. MLP offers the flexibility of creating a custom DL architecture from scratch by combining a different number of hidden layers and nodes. MLP is known for its ability to solve problems stochastically, which often allows approximate solutions for extremely complex problems. MLP is popular due to its fast operation, ease of implementation, and smaller training set requirements \cite{subasi2007eeg}. An MLP architecture consists of three kinds of layers (left to right): input, hidden, and output layers. The hidden layers process and transmit the input information to the output layer. An MLP model with an insufficient or excessive number of neurons in the hidden layer most likely suffers overfitting and lack of generalization. There is no analytical method for determining the number of neurons in the hidden layer. Therefore, it is only found by trial and error \cite{haykin2009neural}. In our case, from $n$ training examples $(\mathcal{H}_1, y_1), (\mathcal{H}_2, y_2),\ldots,(\mathcal{H}_n, y_n)$, a MLP model learns a function $f(\cdot): R^k \rightarrow R^o$, where $k$ is the number of dimensions for input $\mathcal{H} = [c_1, ...,c_{k=|\mathcal{T}|}]$ and $R^o$ is the scalar output $y$. 
%Algorithm \ref{alg:trainmodel} presents the steps of a function \textsc{TrainModel()} that trains the MLP model (i.e., updating the model weights until they convergence).
\end{comment}
\begin{algorithm}[t]  
    \begin{algorithmic}[1]
    \State \ $w \leftarrow (\mathcal{Q}, y)$ \algorithmiccomment{A training workload}
    \State $\mathcal{T} \leftarrow \{t_1,...,\ t_{k}\}$  \algorithmiccomment{A set of $k$ query templates}
    \Function{BinWorkload}{$w$, $\mathcal{T}$}
        \State $Array\ \mathcal{H}[0\ ...\ (k-1)] \leftarrow 0$
        \For{$q_i\ in\ \mathcal{Q}$}
        \State $plan_i$ = getQueryPlan($q_i$)
        \State $features_i$ = getFeatures($plan_i$)
        \State $q_i.template$ = findTemplate($features_i$)
        \EndFor
        \For{$t_j\ in\ \mathcal{T}$}
        \State $\mathcal{H}[j]$ = $countTemplateInstances(t_j, w)$
        \EndFor
        \State \Return $(\mathcal{H}, y)$
    \EndFunction
 %   \State end
  \end{algorithmic}
  \caption{Histogram construction from training workloads}
  \label{algo-kmeans-Templatizing}
\end{algorithm}

%\smallskip

\noindent\textbf{Activation Function}. 
The activation function in each hidden layer determines how the input is transformed. We explored two options: linear and Rectified Linear Unit (ReLU). For simpler datasets with fewer query templates, linear activation performed better, while ReLU proved more effective for complex datasets with more query templates. ReLU enables improved optimization with Stochastic Gradient Descent and efficient computation and is scale-invariant.
\begin{comment}
    

\noindent\textbf{Activation function}. The activation function of each hidden layer controls how the layer's input is transformed. We considered two options for selecting activation functions of our architecture --- a linear activation and a Rectified Linear Unit (ReLU), which is a non-linear activation. Empirically, we observed that with a simpler dataset, which has a smaller number of query templates, the linear activation performed better. However, as the data complexity grows with a larger number of query templates, ReLU appeared to be a better choice. ReLU allows better optimization using Stochastic Gradient Descent and more efficient computation. Also, it's scale-invariant, meaning, its characteristics are not affected by the scale of the input.
\end{comment}
%\smallskip

\noindent\textbf{Loss Function}. Depending on the problem type, an MLP uses different loss functions. For the regression task, we use the mean squared error loss function as follows:
\begin{equation} 
Loss(\hat{y},y,W) = \frac{1}{2N}\sum_{i=1}^N||\hat{y}_i - y_i ||_2^2 + \frac{\alpha}{2N} ||W||_2^2
\end{equation}
where $y_i$ is the target value; $\hat{y}_i$  is the estimated value produced by the MLP model; $\alpha ||W||_2^2$ is an L2-regularization term (i.e., penalty) that penalizes complex models; and $\alpha > 0$ is a non-negative hyperparameter that controls the magnitude of the penalty.
%
The MLP begins with random weights and iteratively updates them to minimize the loss by propagating the loss backward from the output layer to the preceding layers and updating the weights in each layer. The training uses stochastic gradient descent (SGD), where the gradient $\nabla Loss_{W}$ of the loss with respect to the weights is computed and subtracted from $W$. More formally, 
\begin{equation}
W^{i+1} = W^i - \epsilon \nabla {Loss}_{W}^{i}
\end{equation} where $i$ is the iteration step, and $\epsilon$ is the learning rate with a value larger than 0. The algorithm stops after completing a preset number of iterations or when the loss doesn't improve beyond a threshold.

\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{images/LearnedWMP - Constructing Histogram V3.2.png}
  \caption{An example of generating a histogram $\mathcal{H}$ from a training workload $w=(\mathcal{Q}, y)$, where $|\mathcal{Q}|=9$ and $k=4$.}
  %\Description{.}
  \label{fig:binning}
  \vspace{-10px}
\end{figure}

%\smallskip
\noindent\textbf{Optimizer}. We compared L-BFGS \cite{liu1989limited} and Adam \cite{kingma2014adam} optimizers using two datasets --- a small dataset and a relatively large one. 
%Adam is similar to SGD in a sense that it is a stochastic optimizer, but it can automatically adjust the amount to update parameters based on adaptive estimates of lower-order moments.
For the small dataset, L-BFGS was more effective than Adam as it ran faster and learned better model coefficients. In contrast, Adam worked better with the large dataset. Our observation is consistent with {\em scikit-learn}'s \texttt{MLPRegressor}\cite{regressorSklearn}.
%\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.neural_network.MLPRegressor.html}}

\smallskip\noindent\textbf{Hyperparameter Tuning of the MLP Model}. 
To optimize the final model, we tuned hyperparameters, including the number of hidden layers, the number of nodes in each layer, the optimizer, and the dropout rate. Given the large dataset and parameter search space, we employed randomized search, similar to grid search but faster with slightly lower model performance. Using the \texttt{RandomizedSearchCV} method \cite{SklearnSearch} of the \texttt{scikit-learn} library, we found a neural network architecture with eight layers (input, six hidden, and output). The hidden layers contained 48, 39, 27, 16, 7, and 5 nodes from left to right, while the input layer received workload histograms or query distribution, and the output layer provided estimated memory demand.
%\footnote{\url{https://scikit-learn/stable/modules/generated/sklearn.model_selection.RandomizedSearchCV.html}}
%\par \textit{Hyperparameter Tuning of the MLP model:} 
\begin{comment}
    
\smallskip\noindent\textbf{Hyperparameter tuning of the MLP model}. To find an optimum final model, we tuned several hyperparameters, including {\em the number of hidden layers}, {\em the number of nodes in each layer}, {\em the optimizer}, and {\em the dropout rate}. Since we operate on a large dataset and the parameter search space is large (i.e., the combination of different parameter values), we used randomized search to reduce the time for optimizing hyperparameters \cite{bergstra2012random}. The randomized search, which is similar to the grid search, performs a randomized scan of the parameter space. Compared to grid search, randomized search is faster with a slight sacrifice of the model performance. We used the \texttt{RandomizedSearchCV} \footnote{\url{https://scikit-learn/stable/modules/generated/sklearn.model_selection.RandomizedSearchCV.html}} method of the \texttt{scikit-learn} library for random search. For instance, using randomized search with one of our experiment datasets, we came up with a tuned neural network architecture that had eight layers: an {\em input layer}, six {\em hidden layers}, and {\em an output layer}. The input layer receives an input workload, represented as a histogram or a distribution of its queries over query templates; the output layer generates an estimated memory demand for the input workload. Left to right, the hidden layers have 48, 39, 27, 16, 7, and 5 nodes, respectively. 
\end{comment}
 
\smallskip\noindent\textbf{Model Complexity}. Suppose there are $n$ training samples, $k$ features, $l$ hidden layers, each containing $h$ neurons --- for simplicity, and $o$ output neurons. The time complexity of backpropagation is $O (n \cdot k \cdot h^l \cdot o \cdot i)$, where $i$ is the number of iterations. 
%Since backpropagation has a high time complexity, it is advisable to start with smaller number of hidden neurons and few hidden layers for training.

% In this phase, LearnedWMP learns a regression function using the training workloads obtained from step 1. The regression function takes as input a workload, in the form of a distribution of query templates, and computes as output the workload's memory requirement. Though many supervised ML techniques are available to learn this regression function, we are primarily interested in deep neural network (DNN) based architectures for this learning task. DNN recently had several algorithmic breakthroughs and enjoyed remarkable success with many machine learning tasks with unstructured data - image and text \cite{shwartz2021tabular}.  We want to explore if DNN can be useful to learn an accurate non-linear memory estimation function from complex distributions of query templates in the input training workloads. 

% \par \textit{Deep Neural Network (DNN) Architecture:} Several popular DNN architectures exist primarily to work with unstructured input data such as images and text. Unstructured data has a variable-sized input vector and each cell in the vector doesn't carry any meaning on its own \cite{murphy2022probabilistic}. For example, a convolutional neural network (CNN) is used for image recognition tasks where an input image can have different number of pixels than the other images. Also, each pixel in its own doesn't have a meaning. Similarly, recurrent neural network (RNN) and transformers architectures are popular for learning from sequence data of natural languages. Sequences have different sizes, and each word in a sequence doesn't have an independent meaning. In contrast, each of our training workloads has a predefined size of $X \in R^K$, where K is a fixed number of query templates\marin{I think it should be lower case k}. Also, each cell of an input workload vector has a meaning, representing the frequency of a query template. For structured input data, the kind of data we have, a multilayer perceptron (MLP), a particular kind of DNN, is a more promising choice \cite{murphy2022probabilistic}. 
 
%\par \textit{Other Learning Techniques: } 
%\medskip\noindent\textbf{Other machine learning methods}. 
\subsubsection{Other machine learning methods} 
\label{sec:other-ml-methods}
Besides deep learning networks, for a comparative analysis, we explored four additional ML techniques to train \model models. They include a {\em linear} and three {\em tree-based} techniques. For the linear model, we picked \textbf{Ridge}, a popular method for learning regularized linear regression models \cite{raschka2019python}, which can help reduce the overfitting of the linear regression models. From the tree-based approaches, we used \textbf{Decision Tree (DT)}, \textbf{Random Forest (RF)}, and \textbf{XGBoost (XGB)}. %Decision Tree uses a single tree for the prediction task. Random Forest uses an ensemble of trees to compute the final predictions. Each tree split in Random Forest considers only a random subset of the available features. This ensures that the trees in Random Forest are not strongly correlated. Compared to decision trees, Random Forest models have better generalized predictive performance and the ability to handle outliers
DT uses a single tree for predictions, while Random Forest employs an ensemble of trees that consider random feature subsets, resulting in better generalization and outlier handling capabilities \cite{raschka2019python}. 
Our final tree-based model was XGBoost \cite{chen2016xgboost}, a gradient boosting tree technique that has achieved state-of-the-art performance for many machine learning tasks based on tabular data \cite{shwartz2021tabular}. 
%XGBoost creates a sequence of ensemble models, each minimizing the residual errors of the previous model, and generates the final prediction by combining predictions from all models.

%\subsection{Inferencing Stage of the L\MakeLowercase{earned}WMP System}
\subsection{L\MakeLowercase{earned}WMP: Inference Stage}
\label{sec:methodology-inference}

%In Figure \ref{fig:ml-pipeline} (bottom), \texttt{IN1} through \texttt{IN5} correspond to the different steps of the inference stage. Once the model is trained, it can be used to predict the memory usage of an unseen workload $w$, consisting of $\mathcal{Q}$ queries. First, the query plans of the queries $\mathcal{Q}$ in $w$ are collected (\texttt{IN1}), and feature vectors are generated (\texttt{IN2}). Then, each query $q_i \in \mathcal{Q}$ is assigned to a template $t_i \in \mathcal{T}$ (\texttt{IN3}) resulting in the construction of a workload histogram $\mathcal{H}$ (\texttt{IN4}). Finally, given as input the constructed histogram $\mathcal{H}$, the trained model predicts the memory demand $\hat{y}$ of $w$ (\texttt{IN5}).
Algorithm \ref{alg:inference} describes the steps of \textsc{PredictMemory()} function that estimates the memory demand of an unseen workload, $w$. The function operates with two models: a trained $k$-means clustering model, $\mathcal{T}$, which represents a set of learned query templates, and a trained predictive model for estimating workload memory demand. \textsc{PredictMemory()} receives as input an unseen workload whose memory demand needs to be estimated. At \texttt{line 5}, the function generates a histogram vector, $\mathcal{H}$, a distribution of query templates. This step reuses the \textsc{BinWorkload()} function of algorithm \ref{algo-kmeans-Templatizing}. Next, \texttt{line 6} estimates working memory demand $\hat{y}$ of $w$ using $\mathcal{H}$.
\begin{algorithm}[t]
    \begin{algorithmic}[1]
    \State $\mathcal{T} \leftarrow \{t_1,...,\ t_{k}\}$  \algorithmiccomment{A set of $k$ query templates}
    \State $\hat{f}$ \algorithmiccomment{a workload memory estimation function}
    \State $w \leftarrow (\mathcal{Q})$ \algorithmiccomment{An unseen input workload}
    
    \Function{PredictMemory}{$w,\ \mathcal{T},\ \hat{f}$}
       \State $\mathcal{H}$ = $BinWorkload(w, \mathcal{T})$
        \State $\hat{y}$ = $\hat{f}(\mathcal{H})$
        \State \Return $\hat{y}$
    \EndFunction
  %  \State end
    \end{algorithmic}
  \caption{Predict workload memory by rained MLP}
  \label{alg:inference}
\end{algorithm}

==> related.tex <==
%\section{Related Work}
%\label{sec:related}

\noindent Our research relates to machine learning methods for (i) {\em database query optimization} \cite{jarke1984query, ioannidis1996query, chaudhuri1998overview}, (ii) {\em database query resource estimation} \cite{li2012robust}, (iii) {\em query-based workload analysis} \cite{ma2018query}, and (iv) {\em distribution regression problems}. Each of these areas has been under active research for a long time and has broadly related literature. More recently, this kind of literature has been revisited through the lenses of ML. We discuss below some of the most significant research efforts relevant to our work. We cited several related research elsewhere in this paper and will omit repeating them in this section.

%\textbf{ML in the Broader Query Optimization:} 
\subsection{ML for Database Query Optimization} 
In the broader query optimization topic, besides query resource estimation, many recent works explored ML techniques to learn different tasks related to query optimization. Some of the key tasks include cardinality estimation \cite{han2021cardinality, kim2022learned, liu2015cardinality}, query latency prediction \cite{zhou2020query, akdere2012learning}, index selection \cite{sharma2018case, ding2019ai}. A recent cardinality estimation benchmark \cite{han2021cardinality} evaluated eight ML-based cardinality estimation methods---MSCN, LW-XGB, LW-NN, UAE-Q, NeuroCard, BayesCard, DeepDB, and FLAT. Zhou et al. \cite{zhou2020query} proposed a graph-based deep learning method to predict the execution time of concurrent queries. Akdere et al. \cite{akdere2012learning} used support vector machine (SVM) and linear regression to predict the execution time of analytical queries. Marcus and Papaemmanouil \cite{marcus2019plan} proposed a plan-structured neural network architecture, which uses custom neural units designed at the level of query plan operators to predict query execution time. Ahmad et al. \cite{ahmad2011predicting} proposed an ML-based method for predicting the execution time of batch query workloads. They relied upon DBAs to define a set of query types used to create simulated workloads and model interactions among queries. Contender \cite{duggan2014contender} is a framework for predicting the execution time of concurrent analytical queries that compete for I/O.  Ding et al. \cite{ding2019ai} applied machine learning classification techniques to compare the relative cost of a pair of query plans and use that insight in index recommendations.

\begin{figure}[t]
  \includegraphics[width=0.45\textwidth]{images/Batch Sizes V2.png}
  \caption{TPC-DS MAPE at different batch sizes with LearnedWMP XGBoost Model.}
  %\Description{.}
  \label{fig:batchsizes}
  \vspace{-10px}
\end{figure}

%\medskip\noindent\textbf{Histogram construction in DBMS}. 
\subsubsection{Histogram construction in DBMS} 
Our proposed method constructs histograms to represent the workload distribution among query templates. Histograms have played a significant role in estimating query plans cost \cite{bruno2002exploiting}. For an attribute (e.g., the age of a database table), its histogram includes the tuple count and distinct values. During query optimization, the optimizer computes the cost of a candidate plan by referencing attribute histograms in the query expression. These estimates contribute to the overall plan cost, aiding the optimizer in selecting the least expensive plan.
%For an input query expression, when the query optimizer computes the cost of a candidate query execution plan, it looks up the histograms of different attributes of the query expression to estimate the number of tuples the query plan will fetch and process. These estimates contribute to the overall plan cost, aiding the optimizer in selecting the least expensive plan.
% added the fol
%These individual estimates are combined to help estimate the final cost of the plan. Based on the cost estimates, the optimizer chooses the least expensive plan.
% added the following \balance instruction as per this tutorial: https://cs.brown.edu/about/system/managed/latex/doc/balance.pdf (sectopm 3)

\balance

%\textbf{ML for Query Resource Estimation:} 
\subsection{ML for Database Query Resource Estimation} 
Closer to our problem are methods that estimate computing resources---such as memory, CPU, and I/O---for executing database queries. Tang et al. employed machine learning techniques to classify queries into low, medium, and high resource consumption ranges using separate models for memory and CPU, utilizing a bag-of-words approach to extract query keywords as input features and finding XGBoost to be the most accurate model among three compared algorithms \cite{tang2021forecasting}.
%Tang et al. \cite{tang2021forecasting} used ML techniques to classify each query into one of three resource consumption ranges: {\em low}, {\em medium}, and {\em high}. They used two models---one for memory and another for CPU. Using bag-of-words, their method extracted keywords from the query expression and use these as input features to a classification model. They compared three learning algorithms and found an XGBoost model more accurate. 
Ganapathi et al. \cite{ganapathi2009predicting} tried five machine learning techniques to predict run-time resource consumption metrics of individual queries. They achieved the best results with the kernel canonical correlation analysis (KCCA) algorithm. Li et al. \cite{li2012robust} applied boosted regression trees to predict individual queries' CPU and I/O costs. They modeled the resource requirements of each database operator separately by computing a different set of features for each operator type. All the above three approaches \cite{tang2021forecasting, ganapathi2009predicting, li2012robust} generate resource predictions at the level of individual queries. In contrast, our proposed method estimates memory at the level of workload query batches, which we found more accurate and computationally efficient. %%%%HERE \textcolor{red}{
Kipf et al.\cite{kipf2018learned} utilize the Multi-Set Convolutional Network (MSCN) for cardinality estimation, representing query features as sets of tables, joins, and predicates in a query. Similar methods have been used for constructing query-based cardinality estimators. Negi et al.\cite{negi2023robust} introduce techniques for creating sample tables based on join keys (limited to PK-FK joins) and use neural networks to extract information from queries. However, these approaches either involve significant sampling overhead when using samples over joined attributes or rely on static data featurization/samples that are unsuitable for modern databases. Additionally, these methods do not provide explanations for the relationships between data, queries, and actual cardinalities (See Section \ref{sec:evaluation} for our evaluation of the featurization of these models for memory estimation).
%Kipf et. al. [32] concatenate basic relation information and query features together and use a multi-set convolutional neural network to process them and make estimates. , or unrenewable featurization/samples over static data, which are not applicable to dynamic databases. Moreover, these methods do not explain the links among data, queries, and true cardinalities 

\subsection{ML for Query-based Workload Analysis} 
There is a line of research that considers query-based workload analysis. Higginson et al. \cite{higginson2020database} have applied time series analysis, using ARIMA and Seasonal ARIMA (SARIMA), on database workload monitoring data to identify patterns such as seasonality (reoccurring patterns), trends, and shocks. They used these time series patterns in database capacity planning. DBSeer \cite{mozafari2013performance} uses machine learning techniques to predict resource usage metrics, such as CPU, I/O, and memory utilization, of Online Transaction Processing (OLTP) workloads. Each workload is a mixture of different transaction types. DBSeer uses the DBSCAN algorithm on query expressions to learn a set of transaction types. They use linear regression, decision trees, and feedforward neural networks to predict CPU, I/O demand, and memory demand. In comparison, our method doesn't cluster transactions or rely upon query expressions for clustering. Instead, we learn a set of query templates using simple features of the query plan, which we experimentally found to have a stronger correlation with the workload's runtime memory usage. Also, in our experiment, we compared DBSCAN-based templates with $k$-means and found the latter more accurate for resource prediction.
%\textbf{Distribution Regression:} 

\subsection{ML for Distribution Regression Problems}
Distribution regression has emerged as a popular approach in machine learning for mapping complex input probability distributions to real-valued responses, particularly in supervised tasks that require handling input and model uncertainty~\cite{law2018bayesian}.  It stands as a promising alternative to conventional techniques like random forests and neural networks \cite{li2019deep}.
%Distribution regression has recently gained significant attention \cite{law2018bayesian} from the machine learning community for learning a mapping function between complex input probability distributions and the real-valued responses. For supervised machine learning tasks where accounting for input and model uncertainty is important, distribution regression can be a more promising alternative to common ML techniques, such as random forest and neural networks \cite{li2019deep}. 
To the best of our knowledge, we are the first to apply distribution regression to model resource demand forecasting of database workloads. Outside the database domain, some of the illustrative use cases of distribution regression include predicting health indicators from a patient's list of blood tests \cite{mao2022coefficient}, solar energy forecasting \cite{li2019deep}, and traffic prediction \cite{li2019deep}. Many recent papers have offered approaches and optimization techniques for solving distribution regression tasks. Law et al. \cite{law2018bayesian} offered a Bayesian-based method to account for uncertainty in both the input and the output of a distribution regression task. Li et al. \cite{li2019deep} re-framed the task of predicting a single real-value response to a multi-class classification task using distribution regression. Mao et al. \cite{mao2022coefficient} proposed a coefficient-based regularized method for learning distribution regression functions using indefinite kernels.

